Structural Patterns and Generative Models of Real-world Hypergraphs

Graphs have been utilized as a powerful tool to model pairwise relationships between people or objects. Such structure is a special type of a broader concept referred to as hypergraph, in which each hyperedge may consist of an arbitrary number of nodes, rather than just two. A large number of real-world datasets are of this form - for example, list of recipients of emails sent from an organization, users participating in a discussion thread or subject labels tagged in an online question. However, due to complex representations and lack of adequate tools, little attention has been paid to exploring the underlying patterns in these interactions. In this work, we empirically study a number of real-world hypergraph datasets across various domains. In order to enable thorough investigations, we introduce the multi-level decomposition method, which represents each hypergraph by a set of pairwise graphs. Each pairwise graph, which we refer to as a k-level decomposed graph, captures the interactions between pairs of subsets of k nodes. We empirically find that at each decomposition level, the investigated hypergraphs obey five structural properties. These properties serve as criteria for evaluating how realistic a hypergraph is, and establish a foundation for the hypergraph generation problem. We also propose a hypergraph generator that is remarkably simple but capable of fulfilling these evaluation metrics, which are hardly achieved by other baseline generator models.

==> 000abstract.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \comment{test}


Graphs have been utilized as a powerful tool to model relationships between people and objects. A special type of this structure is hypergraph, in which each hyperedge, which is an extension of the usual notation of edge, may consist of an arbitrary number of nodes. A large number of real-world datasets are demonstrated in this form – for example, lists of recipients of emails sent from an organization, users participating in a discussion thread or subject labels tagged in an online question. However, due to complex representations and lack of adequate tools, little attention has been paid to exploring the underlying patterns in these interactions.

In this work, we empirically study a number of real-world hypergraph datasets across various domains. We find that with proper interpretations, the investigated hypergraphs obey a consistent set of several properties as well as small-world phenomena. The characteristics serve as criteria for evaluating how \textit{realistic} a hypergraph is, and establish the ground for the hypergraph generation problem. We also propose a simple hypergraph generator, yet capable of fulfilling these evaluation metrics, which are hardly achieved by other baseline generator models.



==> 030method.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\notice{{\em novelty}: NO citations, outside the 'survey'  - 
they make \method seem incremental. }


In this section we present the proposed method,
we analyze it and provide the reader with several interesting -at least in our opinion-
observations. Table~\ref{tab:dfn} gives the list of symbols we use.
\notice{Give table of symbols and dfns}

\begin{table}[htbp]
\begin{center}


\begin{tabular}{|c|c|}
\hline  
Symbols & Definitions \\ 
\hline
$G$  & a graph \\ 
\hline  
$A$  &  adjacency matrix\\ 
\hline 
\end{tabular} 
\caption{Symbols and Definitions \label{tab:dfn}}
\end{center}
\end{table}


\subsection{Intuition}
The main idea behind our \method is to exploit network effects:
if we see a bi-partite core, then we suspect fraud.

Figure \ref{fig:tikz} and \ref{fig:tikz2} illustrates the intution
\reminder{comment them out, if the tikz package is missing}

\begin{figure}[htbp]
\begin{centering}
    % if tikz is missing, comment out all the lines below % 'tikz comment out'
    \input{FIG-TIKZ/sample-fig-tikz.tex}
\caption{Sample tikz figure \label{fig:tikz}}
\end{centering}
\end{figure}

\begin{figure}[htbp]
\begin{centering}
    % if tikz is missing, comment out all the lines below % 'tikz comment out'
    \input{FIG-TIKZ/sample-fig-tikz2.tex}
\caption{Another Sample tikz figure \label{fig:tikz2}}
\end{centering}
\end{figure}


\subsection{Algorithm}
% \reminder{details on the algorithm(s)}

Algorithm~\ref{algo:main} shows the pseudo code
and Algorithm~\ref{algo:sample} shows a variation


% \begin{algorithm}[H]
% needs \usepackage{algorithm2e}
\begin{algorithm}[htbp]
% \SetAlgoVlined
\SetAlgoLined
% \SetNoLine
\LinesNumbered
\KwData{a graph $G$}
\KwResult{the communities in $G$}
initialization\;
put graph $G$ on stack\;
pop stack\;
\While{stack is not empty}{
   process current graph\;
   % \eIf(\tcp{clique}){has $n^2$ edges}{
   \eIf{has $n^2$ edges}{
      add to output\;
   }{
      split in two\;
      put both on stack\;
   }
   pop stack\;
}

\caption{FakeCom: Community detection algorithm \label{algo:main}}
\end{algorithm}

\begin{algorithm}[h]
% \SetAlgoLined
\SetAlgoVlined
\KwData{this text}
\KwResult{how to write algorithm with \LaTeX2e }
initialization\;
\While{not at end of this document}{
read current\;
\eIf(\tcp{nice!}){understand}{
go to next section\;
current section becomes this one\;
}{
go back to the beginning of current section\;
}
}
\caption{How to write algorithms\label{algo:sample}}
\end{algorithm}

\subsection{Complexity Analysis}
\begin{theorem}
\method requires time linear on the input size
\end{theorem}

\begin{proof}
from Eq *bla*, with lagrange multipliers
\end{proof}


\subsection{SQL implementation}
In fact, we can use SQL to implement our algorithm:
\lstset{language=sql, numbers=left, numberstyle=\tiny}
\begin{lstlisting}
select name, ssn
from student
where name = 'smith'
  and grade = 'A';
\end{lstlisting}







==> 040experiment.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Here we report experiments to answer the following questions
\notice{{\em ``bullets''}: should correspond to the 'advantages' bullets
in the intro and conclusions, as well as
to the headers of the upcoming subsections}



% A better way to create tight lists:
% \begin{compactitem}
% \item first item
% \item second itm
% \end{compactitem}


\begin{compactenum}[{Q}1.]
\item {\bf \scale}: How fast is our \method

\item {\bf \effective}: How well does \method work on real data?

\reminder{\item some other question, if any}
% {\bf Accuracy}: How well can it reconstruct the actual values

\end{compactenum}

The graphs we used in our experiments are described in the table~\ref{tab:datasets}.

%\reminder{old stuff - usepackage paralist, above, instead}
%
%\begin{enumerate*}
%\item Q1 - scalability: how fast is \method?
%\item Q2 - effectiveness: how effective is \method?
%\item Q3: \reminder{some other question}
%\end{enumerate*}


\begin{table*}[ht]
\begin{center}
\begin{tabular}{r|r|l}
   Nodes & Edges & Description  \\ \hline \hline
  \multicolumn{3}{l}{\textbf{Real-world Networks}} \\ \hline \hline 
  13,579 & 37,448 & AS Oregon \\  % AsRouteViews
  23,389 & 47,448 & CAIDA AS 2004 to 2008  \\
  \hline \hline
\end{tabular}
\end{center}
\caption{Summary of real-world networks used.}
\label{tab:datasets}
\end{table*}

\subsection{Q1 - \scale }

In figure~\ref{fig:zooming} 
\notice{{\em 2-word-tag:} For each caption, give a 2-3 word summary.}
we present the experimental results for
the real-world datasets we used. 

\begin{figure}[hbtp]
\centering
\includegraphics[width=0.4\textwidth]{FIG/scale.png}
\caption{{\bf  \method scales lineary}: response time vs input size \label{fig:zooming}}
\end{figure}


\subsection{Q2 - \effective}

In Figure bla, we show the precision/recall of \method for the epinions.com dataset.
Notice that \reminder{the results are great}

\subsection{Discussion - practitioner's guide}
Given the above, we recommend that practitioners choose \reminder{bla} for
the parameter values of \method, and \reminder{do preprocessing using bla-bla}
for their datasets.

\subsection{Discoveries - \method at work}
Thanks to our method, we processed real data
and noticed the following  observations 
\notice{{\em success stories:} elaborate... -
if too many nice observations, promote this to a full section}
\begin{observation}
\method works better than expected, on real data
\end{observation}
The reason is that we assumed uniformity,
while real data have skewed distributions (Pareto-like),
and thus favor our approach.

\begin{observation}
\method works faster than expected
\end{observation}
bla-bla




==> 040observation_backup.tex <==
In this section, we demonstrate that, at each level of decomposed graphs of real hypergraphs, the following general patterns hold:
\begin{itemize}[$\bullet$]
	\item {\bf P1.} \connectcomp %The decomposed graph has a giant connected component.
	\item {\bf P2.}  \degdistr %The decomposed graph has a heavy-tailed distribution in degrees.
	\item {\bf P3.}  \effdiam %The decomposed graph has a small effective diameters.
	\item {\bf P4.}  \clustcoef %The decomposed graph has a high global clustering coefficient.
	\item {\bf P5.} \sngvals %The decomposed graph has a skewed distribution of singular values.
\end{itemize}
We examine \textbf{thirteen} real hypergraph datasets of medium to large sizes. Details on the datasets can be found in Appendix~\ref{appendix:description}.



\subsection{Details on Patterns}
\label{sec:exp:patterns:detail}
%\reminder{old stuff - usepackage paralist, above, instead}
%
%\begin{enumerate*}
%\item Q1 - scalability: how fast is \method?
%\item Q2 - effectiveness: how effective is \method?
%\item Q3: \reminder{some other question}
%\end{enumerate*}

There are some details worth mentioning for the patterns.

\smallsection{Null model: Random Hypergraphs (Null.).} We use a random hypergraph corresponding to each real hypergraph as the null model. Specifically, given a hypergraph, the null model is constructed by randomly choosing nodes to be contained in each hyperedge, while keeping its original size.

\smallsection{Giant connected component.} This property means that there is a connected component comprising of a large proportion of nodes, and this proportion is significantly larger (specifically, at least $70$ times larger) than that of the second largest connected component. This property serves as a basis for the other properties. For example, without a giant connected component (i.e, the graph is ``shattered'' into small connected communities), %degree distribution would not be heavy-tailed (KJ: is it true?), and  
diameter would clearly be small as a consequence, not as an independent property of the dataset.

\smallsection{Heavy-tailed degree distribution}: The degree of a node is defined as the number of its neighbors. This properties means that the degree distribution is heavy-tailed, i.e decaying at a slower rate than the exponential distribution (exp.). Apart from visual inspection, we confirm this property by the following 2 steps:
\begin{itemize}[$\bullet$]
\item Lilliefors test \cite{lilliefors1969kolmogorov} is applied at significance level $2.5\%$ with the null hypothesis $H_{0}$ that the given distribution follows exp.
\item The likelihood method in \cite{clauset2009power, alstott2014powerlaw} is used on the given distribution to compute the likelihood ratio $r$ of a heavy-tailed distribution (power-law, truncated power-law or lognormal) against exp. If $r>0$, the given distribution is more similar to a heavy-tailed distribution than exp.
\end{itemize}
In all cases, either $H_{0}$ is rejected or $r>0$ (both claims hold in most cases), indicating evidence for heavy-tailed degree distribution.

\smallsection{Small diameter.} Graphs in networks are usually not completely connected, which makes diameter subtle to define. 
We adopt the definition in \cite{leskovec2005graphs}, where diameter is the minimum distance $d$ such that approximately $90 \%$ of all connected pairs are reachable by a path of length at most $d$. 
This property means that the diameter in real datasets is relatively small with respect to the number of nodes.
Note that the null model also possesses this characteristic, %at the node-level decomposition, 
and comparing real-world datasets and the corresponding null model in this aspect does not yield consistent results. 

\smallsection{High clustering coefficients.} We make use of the global clustering coefficient $C$, defined as the ratio of closed triangles (i.e., cliques of size $3$):
 $$C := 3\times \frac{\text{the number of triangles in the network}}{\text{the number of connected triples of nodes}}$$
This property means that this statistic in the real datasets is significantly larger than that in the corresponding null models.

\smallsection{Skewed singular values}: This property means the singular-value distribution is usually heavy-tailed and it is verified in the same manner as the pattern \textbf{P2}.

\input{046cshatterlevel.tex}
% table of node-level properties
\input{041cnodeproperties.tex}
% figure of singular values distribution of node-level
%\begin{figure*}[t]
%	\vspace{-2mm}
%	\begin{center}
%		\begin{tabular}{cccc}
%			\includegraphics[width=1.65in]{FIG/Real/nodesng_coauth-History.png} &
%			\includegraphics[width=1.65in]{FIG/Real/nodesng_email-Eu.png} &
%			%(a) coauth-DBLP  & (b) NDC-classes   \\
%			\includegraphics[width=1.65in]{FIG/Real/nodesng_NDC-substances.png} &
%			\includegraphics[width=1.65in]{FIG/Real/nodesng_tags-math.png} \\
%			%(c) tags-stack-overflow  & (d) threads-math  \\
%		\end{tabular}
%		\caption{\label{fig:node_singular} Singular-value distributions of \%textit{\nodeproj}.
%			The singular values are skewed, following near power-law distributions, i.e., they form a nearly straight line in the log-log scale. }
%	\end{center}
%\end{figure*}

Since these properties are defined on pairwise graphs, we examine them in decomposed graphs of each original hypergraph, which are based on pairwise edges. \blue{By our definition, a hyperedge of size $n > k$ results in ${n}\choose{k}$ nodes and ${{n}\choose{k}}\choose{2}$ edges in the $k$-level decomposed graph. For example, a hyperedge of 8 nodes is decomposed into ${8}\choose{3}$ $= 56$ nodes and ${56}\choose{2}$ $= 1,540$ edges in the triangle-level decomposed graph. 
In order to avoid dominance by the edges resulted from  large-size hyperedges, in the node-level decomposed graphs, only hyperedges with up to 25 nodes are considered.
In higher-level decomposition, we only consider hyperedges with up to $7$ nodes. Note that, in each dataset, the vast majority of hyperedges consist of $7$ or less nodes.}

%\kijung{It is unclear what ``dominance'' means. By our definition, a hyperedge of \blue{size $n > k$ results in a clique of size ${n}\choose{k}$ in the $k$-level decomposed graph....}}
%\kijung{It would be better if we used hyperedges of sizes up to 7 nodes consistently in all levels...}



\subsection{Node-level decomposed graph}
Consider the coauthorship data as an example: in our node-level decomposed graph, each node represents an author, and two nodes are connected if and only if these two authors have coauthored at least one paper before. 
Therefore, this node-level decomposition can be interpreted as an author network. 
Such node-level decomposed graphs are not  ``real'' graphs since they are obtained by decomposing the original hypergraphs.
However, they represent pairwise relationships as real-world graphs do, and by this interpretation, we deduce that the node-level decomposed graphs of real-world hypergraphs will exhibit the five patterns (i.e., P1-P5), which are well-known for real-world graph \cite{leskovec2005graphs, leskovec2005realistic, faloutsos1999power,broder2000graph,milgram1967small, albert1999internet, bollobas2004diameter,yin2017local, kumar2000stochastic}.
%(please do some referencing here, you can copy references from Kronecker and GraphsoverTime).)


\input{047summary_degrees_sng_figure.tex}
%\input{047summary_degrees_figure.tex}
%\input{047summary_degrees_figure_.tex}

In the following subsections, in order to facilitate our investigation of high-order interactions among nodes, we consider higher levels of decomposition, in which a node can be a group of 2,3 or 4 nodes in the original hypergraph.
We observe that the levels of such high-order interactions vary among datasets, as summarized in Table~\ref{tab:gcc}.
% This statement is about some datasets shattered at edge, some at triangle, some still survive at 4-clique.

\input{048summary_properties.tex}
%\input{043edgeproperties.tex}
\subsection{Edge-level decomposed graph}
From this level, the decomposed graph of the \textit{null model} is almost shattered into small isolated cliques. 
As a result, the clustering coefficient is unrealistically high, making it no longer valid to compare this statistic to that of the real-world edge-level decompositions.

The \edgeproj of $11$ (out of $13$) datasets still retain the five structural patterns of real-world graphs (i.e., P1-P5).

There is a strong positive correlation between the distribution of hyperedge sizes and whether the graph is shattered at edge-level decomposition. Take the proportion of unique hyperedges of sizes at most $2$ as the feature. Datasets with this feature greater than $75\%$ are shattered, and the others retain giant connected components. 


\subsection{Triangle-level decomposed graph}
%As claimed in \cite{benson2018simplicial}, the triangle is the most simple type of high-order level interaction in hypergraphs. Here, we investigate such structure, but in a different approach.
%By decomposing the hypergraphs onto the triangle-level, in which we treat each group of 3 nodes, which forms a triangle in the \nodeproj, as a \text{triangle-level node}. 
At the triangle-level, $6$ (out of $13$) datasets have giant connected components, and the previously mentioned properties are observable in them.
We only report the properties of the datasets with giant connected components since the other statistics are not meaningful in datasets almost shattered into small isolated connected components.

Except for \textit{email-Eu} and \text{NDC-classes}, datasets having proportion of hypergedges of sizes at most 3 larger than $60\%$ are shattered at this level, otherwise they possess a giant connected component.


\subsection{4clique-level decomposed graph}
While most of the hypergraphs are shattered into isolated cliques at this decomposition level, $5$ (out of $13$) datasets  still have giant connected component and exhibit the common properties of real-world graphs.
There is no evidence for correlation between the distribution of hyperedge sizes and whether the hypergraph is shattered at this level.

% figure of degree distribution of 4clique-level
%\begin{figure}[!tp]
%\begin{center}
%  \begin{tabular}{cc}
%    \includegraphics[width=1.5in]{FIG/Real/4cliqueDeg_DAWN.png} &
%    \includegraphics[width=1.5in]{FIG/Real/4cliqueDeg_tags-ask-ubuntu.png} \\
%    %(a) DAWN  & (b) email-Eu   \\
%    \includegraphics[width=1.5in]{FIG/Real/4cliqueDeg_tags-math.png} &
%    \includegraphics[width=1.5in]{FIG/Real/4cliqueDeg_tags-stack-overflow.png} \\
%    %(c) tags-ask-ubuntu  & (d) tags-stack-overflow  \\
%  \end{tabular}
%  \caption{\label{fig:4clqiue_degree} Degree distributions of the \textit{\fcliqueproj}. These datasets, which maintain a giant connected component at this decomposition level, also maintain heavy-tailed degree distributions.
%%  Heavy-tailed degree distribution are heavy tailed. 
%  %log-log scaled degree distribution resembles a straight line going downward, revealing a power-law distribution. %\kijung{Please summarize our observation regarding this figure. make sure that this figure is mentioned in the text.}
%  }
%\end{center}
%\end{figure}

The empirical data support our claims in Sects. 4.2-4.4, as seen in Tables~\ref{tab:node_properties},\ref{tab:edge_triangle_4clique_properties} and Fig.~\ref{fig:summary_degree_sng_figure}. Due to the space limit, only some representative results are highlighted. The complete set of figures, numerical data, and loglikehood ratios (Sect.~\ref{sec:exp:patterns:detail}) can be found in the online appendix \cite{appendix}. As most hyperedges are of sizes only up to 4, considering interactions of subsets of sizes at least 5 would omit most of the hyperedges. Thus, we only investigate up to the 4clique level.   

==> 045fourcliqueproperties.tex <==
\begin{table}[t]
%\setlength{\tabcolsep}{1.8pt}
\centering
\caption{\label{tab:fourclique_properties}Numerical properties of \textit{\fcliqueproj} of the datasets. These five datasets have the highest strength of high-order interactions. Size-4 group interactions are sufficiently strong to yield a relatively small diameter, high clustering coefficient in a giant connected component. Datasets shattered without giant connected components are omitted in the table.}
\scalebox{1}{
\begin{tabular}{l|cccc}
\toprule
Measure                & Nodes    & Connect.   &Eff.    & Clust.    \\
&          & Comp.      & Diam.  & Coeff. 
\\ \midrule
\multicolumn{4}{l}{\textbf{Real-world Hyper-graphs}} \\ 
\midrule
DAWN                   & 284,755    & 0.52      & 8.1        & 0.89		  \\
email-Eu               & 24,772     & 0.41      & 15.3       & 0.89		  \\
%NDC-classes            & 3,078      & 0.19      & 2.7   	    & 0.96		  \\
tags-ask-ubuntu        & 145,676    & 0.22      & 17.1       & 0.74		  \\
tags-math              & 156,129    & 0.35      & 14.8       & 0.71		  \\
tags-stack-overflow    & 7,887,748   & 0.42      & 13         & 0.76		  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summaryDAWN_clust.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summaryDAWN_connect.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_DAWN} Proportion of nodes in the largest connected component pattern of the \textit{DAWN} dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level  & Real      & {\bf \generator}     & Naive         & Subset\\ 
       & Data      & {\bf (Proposed)}     & PA            & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node      & 0.89     & 0.996              &  0.73         & 0.999           \\
edge      & 0.98     & 0.98               &  0.95         & 0.95			  \\
triangle  & 0.91     & 0.89               &  \red{0.08}   &  0.79			  \\
4clique   & 0.52     & 0.81               &  \red{0.01}   & 0.22      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summaryDAWN_diameter.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summaryemail-Eu_clust.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summaryemail-Eu_connect.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_email-Eu} Proportion of nodes in the largest connected component pattern of the \textit{email-Eu} dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level        & Real        & {\bf \generator}     & Naive       & Subset\\ 
             & Data        & {\bf (Proposed)}     & PA          & Sampling \\
\midrule 
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node         & 0.98        & 0.995                &  0.997       & 0.988           \\
edge         & 0.98        &  0.86                &  0.935       & 0.8			  \\
triangle     & 0.87        &  0.86                &  0.54        &  0.5			  \\
4clique      & 0.41        &  0.76                &  \red{0.03}  & \red{0.04}	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summaryemail-Eu_diameter.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summarytags-ask-ubuntu_clust.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summarytags-ask-ubuntu_connect.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the \textit{tags-ask-ubuntu} dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summarytags-ask-ubuntu_diameter.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summarytags-math_clust.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                            
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summarytags-math_connect.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-math} Proportion of nodes in the largest connected component pattern of the \textit{tags-math} dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level    & Real      & {\bf \generator}         & Naive            & Subset\\ 
         & Data      & {\bf (Proposed)}         & PA               & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node     & 0.998     & 0.997                    &  0.997            & 0.996           \\
edge     & 0.995     & 0.98                     &  0.993            & 0.97			  \\
triangle & 0.91      & 0.81                     &  0.77             &  0.55			  \\
4clique  & 0.35      & 0.28                     &  0.12            & \red{0.02}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> 091summarytags-math_diameter.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}

==> summary_number_patterns.tex <==
\begin{table}[t]
\begin{center}
\caption{\label{tab:counts} Number of patterns reproduced by each generator. In order to learn $S$, $NP$ and $n$, we used the datasets that exhibit the patterns most clearly, i.e., those with all $20$ patterns ($4$ decomposition levels $\times$ $5$ patterns). \generator, our proposed hypergraph generator, reproduced most patterns.
}
\begin{tabular}{l|c|ccc}
\toprule
 & Real    & {\bf HyperPA} & Naive  & Subset  \\ 
Dataset  & Data& {\bf (Proposed) }  & PA & Sampling \\
\midrule  
        tags-ask-ubuntu     & 20 & \textbf{20} & 17 & 16  \\ 
        tags-math           & 20 & \textbf{20} & 17 & 17  \\ 
        DAWN                & 20 & \textbf{19} & 8 & \textbf{19}  \\
        email-Eu            & 20 & 15         & 12  & \textbf{16}  \\ 
\bottomrule
\end{tabular} 
\end{center}
\end{table}

==> summarytags-ask-ubuntu_connect.tex <==
% table of survival
\begin{table}[tb]
%\setlength{\tabcolsep}{1.5pt}
\centering
\caption{\label{tab:gcc_tags-ask-ubuntu} Proportion of nodes in the largest connected component pattern of the  tags-ask-ubuntu dataset and the corresponding synthetic hypergraphs produced by three generators. \textit{Subset Sampling} failed to recapture the strength of size-4 group interactions as its \fcliqueproj is shattered, while in the real dataset, a giant connected component is still present at this level.}
\scalebox{1}{
\begin{tabular}{l|c|ccc}
\toprule
Level & Real      & {\bf \generator}     & Naive  & Subset\\ 
& Data & {\bf (Proposed)} & PA & Sampling \\
\midrule
%\multicolumn{4}{l}{\textbf{tags-ask-ubuntu}} \\  \midrule                       
node            & 0.99     & 0.99   &  0.99   & 0.99           \\
edge     & 0.98     & 0.92   &  0.98   & 0.95			  \\
triangle     & 0.79     & 0.81   &  0.74   &  0.55			  \\
4clique       & 0.21     & 0.39   &  0.11   & \red{0.002}      	  \\
\bottomrule
\end{tabular}
}
\end{table}
